Shortcut Learning in Binary Classifier Black Boxes: Applications to Voice Anti-Spoofing and Biometrics

The widespread adoption of deep-learning models in data-driven applications has drawn attention to the potential risks associated with biased datasets and models. Neglected or hidden biases within datasets and models can lead to unexpected results. This study addresses the challenges of dataset bias and explores ``shortcut learning'' or ``Clever Hans effect'' in binary classifiers. We propose a novel framework for analyzing the black-box classifiers and for examining the impact of both training and test data on classifier scores. Our framework incorporates intervention and observational perspectives, employing a linear mixed-effects model for post-hoc analysis. By evaluating classifier performance beyond error rates, we aim to provide insights into biased datasets and offer a comprehensive understanding of their influence on classifier behavior. The effectiveness of our approach is demonstrated through experiments on audio anti-spoofing and speaker verification tasks using both statistical models and deep neural networks. The insights gained from this study have broader implications for tackling biases in other domains and advancing the field of explainable artificial intelligence.

==> tables/definition_config.tex <==
\begin{table}[!t]
    \caption{We consider \emph{biased} audio anti-spoofing task with two classes (spoof and bona fide) where specific interventions are applied to one of the four data subsets as indicated. %The binary flags \texttt{0} and \texttt{1} indicate whether or not the specific subset undergoes perturbation. 
    Besides the original dataset protocol (\textbf{O}) without interventions, we consider four biased configurations labeled $\textbf{A}$ through $\textbf{D}$. In \textbf{A} and \textbf{B}, the treatment for the same class across training and test subsets are identical; in \textbf{C} and \textbf{D}, the treatments are flipped. Training and evaluating models on biased data allows addressing their sensitivity to unintended `shortcuts'. We expect a model to yield \emph{lower} error rates on $\textbf{A}$ and $\textbf{B}$ compared to $\textbf{O}$; and \emph{higher} error rate on $\textbf{C}$ and $\textbf{D}$ compared to $\textbf{O}$.} 
    \label{tab:config}
    %\label{tab:subset-perturbation-specifications}
    \centering
    \begin{tabular}{|l||c|c|c|c|}
         \hline
          \textbf{Configuration} & \multicolumn{2}{c}{Train} & \multicolumn{2}{|c|}{Test} \\
        \cline{2-5}
         \texttt{(indicator)} & Spf & Bona & Spf & Bona \\
         \hline
         \textbf{O} \texttt{(0 0 0 0)} &  &  &  & \\
         \hline
         \textbf{A} \texttt{(0 1 0 1)} &  & \checkmark &  & \checkmark \\
         \textbf{B} \texttt{(1 0 1 0)} & \checkmark &  & \checkmark &\\
         \hline
         \textbf{C} \texttt{(0 1 1 0)} & & \checkmark & \checkmark & \\
         \textbf{D} \texttt{(1 0 0 1)} & \checkmark &  & & \checkmark \\
    \hline
    \end{tabular}
\vspace{-15pt}
\end{table}

==> tables/intervention_blanking.tex <==
\begin{comment}
    

\begin{table*}[]
  \centering
  \scriptsize
  \caption{Model parameters for nonspeech blanking intervention.}
  \label{tab:interventionblanking}
  \setlength{\tabcolsep}{0.5em}
\begin{tabular}{l|cccccccccccc|cccccccccccc|}
\cline{2-25}
 & \multicolumn{12}{c|}{\textbf{GMM}} & \multicolumn{12}{c|}{\textbf{AASIST+RawBoost}} \\ \hline
\multicolumn{1}{|l|}{Params.} & \multicolumn{1}{c|}{\textbf{O}} & \multicolumn{1}{c|}{\textbf{I}} & \multicolumn{1}{c|}{$\textbf{M}_{tr}$} & \multicolumn{1}{c|}{$\textbf{M}_{te}$} & \multicolumn{1}{c|}{$\textbf{IT}_{b}$} & \multicolumn{1}{c|}{$\textbf{IT}_{s}$} & \multicolumn{1}{c|}{$\textbf{IV}_{bs}$} & \multicolumn{1}{c|}{$\textbf{IV}_{sb}$} & \multicolumn{1}{c|}{$\textbf{O}_{s}$} & \multicolumn{1}{c|}{$\textbf{O}_{b}$} & \multicolumn{1}{c|}{$\textbf{I}_{s}$} & $\textbf{I}_{b}$ & \multicolumn{1}{c|}{\textbf{O}} & \multicolumn{1}{c|}{$\textbf{I}$} & \multicolumn{1}{c|}{$\textbf{M}_{tr}$} & \multicolumn{1}{c|}{$\textbf{M}_{te}$} & \multicolumn{1}{c|}{$\textbf{IT}_{b}$} & \multicolumn{1}{c|}{$\textbf{IT}_{s}$} & \multicolumn{1}{c|}{$\textbf{IV}_{bs}$} & \multicolumn{1}{c|}{$\textbf{IV}_{sb}$} & \multicolumn{1}{c|}{$\textbf{O}_{s}$} & \multicolumn{1}{c|}{$\textbf{O}_{b}$} & \multicolumn{1}{c|}{$\textbf{I}_{s}$} & $\textbf{I}_{b}$ \\ \hline
\multicolumn{1}{|l|}{$\mu$} & \multicolumn{1}{c|}{12.23} & \multicolumn{1}{c|}{22.49} & \multicolumn{1}{c|}{44.83} & \multicolumn{1}{c|}{0.00} & \multicolumn{1}{c|}{0.00} & \multicolumn{1}{c|}{99.99} & \multicolumn{1}{c|}{97.85} & \multicolumn{1}{c|}{4.01} & \multicolumn{1}{c|}{61.26} & \multicolumn{1}{c|}{26.06} & \multicolumn{1}{c|}{26.06} & \multicolumn{1}{c|}{26.06} & \multicolumn{1}{c|}{3.12} & \multicolumn{1}{c|}{2.31} & \multicolumn{1}{c|}{3.71} & \multicolumn{1}{c|}{0.88} & \multicolumn{1}{c|}{0.52} & \multicolumn{1}{c|}{35.96} & \multicolumn{1}{c|}{36.03} & \multicolumn{1}{c|}{36.03} & \multicolumn{1}{c|}{1.62} & \multicolumn{1}{c|}{3.96} & \multicolumn{1}{c|}{3.51} & \multicolumn{1}{c|}{26.06} \\ \hline
\multicolumn{1}{|l|}{$d$} & \multicolumn{1}{c|}{12.23} & \multicolumn{1}{c|}{22.49} & \multicolumn{1}{c|}{44.83} & \multicolumn{1}{c|}{0.00} & \multicolumn{1}{c|}{0.00} & \multicolumn{1}{c|}{99.99} & \multicolumn{1}{c|}{97.85} & \multicolumn{1}{c|}{4.01} & \multicolumn{1}{c|}{61.26} & \multicolumn{1}{c|}{26.06} & \multicolumn{1}{c|}{26.06} & \multicolumn{1}{c|}{26.06} & \multicolumn{1}{c|}{3.12} & \multicolumn{1}{c|}{2.31} & \multicolumn{1}{c|}{3.71} & \multicolumn{1}{c|}{0.88} & \multicolumn{1}{c|}{0.52} & \multicolumn{1}{c|}{35.96} & \multicolumn{1}{c|}{36.03} & \multicolumn{1}{c|}{36.03} & \multicolumn{1}{c|}{1.62} & \multicolumn{1}{c|}{3.96} & \multicolumn{1}{c|}{3.51} & \multicolumn{1}{c|}{26.06} \\ \hline
\multicolumn{1}{|l|}{$\beta_{\mathrm{spoof}}$} & \multicolumn{1}{c|}{12.23} & \multicolumn{1}{c|}{22.49} & \multicolumn{1}{c|}{44.83} & \multicolumn{1}{c|}{0.00} & \multicolumn{1}{c|}{0.00} & \multicolumn{1}{c|}{99.99} & \multicolumn{1}{c|}{97.85} & \multicolumn{1}{c|}{4.01} & \multicolumn{1}{c|}{61.26} & \multicolumn{1}{c|}{26.06} & \multicolumn{1}{c|}{26.06} & \multicolumn{1}{c|}{26.06} & \multicolumn{1}{c|}{3.12} & \multicolumn{1}{c|}{2.31} & \multicolumn{1}{c|}{3.71} & \multicolumn{1}{c|}{0.88} & \multicolumn{1}{c|}{0.52} & \multicolumn{1}{c|}{35.96} & \multicolumn{1}{c|}{36.03} & \multicolumn{1}{c|}{36.03} & \multicolumn{1}{c|}{1.62} & \multicolumn{1}{c|}{3.96} & \multicolumn{1}{c|}{3.51} & \multicolumn{1}{c|}{26.06} \\ \hline
\multicolumn{1}{|l|}{$\beta_{\mathrm{bona}}$} & \multicolumn{1}{c|}{12.23} & \multicolumn{1}{c|}{22.49} & \multicolumn{1}{c|}{44.83} & \multicolumn{1}{c|}{0.00} & \multicolumn{1}{c|}{0.00} & \multicolumn{1}{c|}{99.99} & \multicolumn{1}{c|}{97.85} & \multicolumn{1}{c|}{4.01} & \multicolumn{1}{c|}{61.26} & \multicolumn{1}{c|}{26.06} & \multicolumn{1}{c|}{26.06} & \multicolumn{1}{c|}{26.06} & \multicolumn{1}{c|}{3.12} & \multicolumn{1}{c|}{2.31} & \multicolumn{1}{c|}{3.71} & \multicolumn{1}{c|}{0.88} & \multicolumn{1}{c|}{0.52} & \multicolumn{1}{c|}{35.96} & \multicolumn{1}{c|}{36.03} & \multicolumn{1}{c|}{36.03} & \multicolumn{1}{c|}{1.62} & \multicolumn{1}{c|}{3.96} & \multicolumn{1}{c|}{3.51} & \multicolumn{1}{c|}{26.06} \\ \hline
\multicolumn{1}{|l|}{$\sigma$} & \multicolumn{1}{c|}{12.23} & \multicolumn{1}{c|}{22.49} & \multicolumn{1}{c|}{44.83} & \multicolumn{1}{c|}{0.00} & \multicolumn{1}{c|}{0.00} & \multicolumn{1}{c|}{99.99} & \multicolumn{1}{c|}{97.85} & \multicolumn{1}{c|}{4.01} & \multicolumn{1}{c|}{61.26} & \multicolumn{1}{c|}{26.06} & \multicolumn{1}{c|}{26.06} & \multicolumn{1}{c|}{26.06} & \multicolumn{1}{c|}{3.12} & \multicolumn{1}{c|}{2.31} & \multicolumn{1}{c|}{3.71} & \multicolumn{1}{c|}{0.88} & \multicolumn{1}{c|}{0.52} & \multicolumn{1}{c|}{35.96} & \multicolumn{1}{c|}{36.03} & \multicolumn{1}{c|}{36.03} & \multicolumn{1}{c|}{1.62} & \multicolumn{1}{c|}{3.96} & \multicolumn{1}{c|}{3.51} & \multicolumn{1}{c|}{26.06} \\ \hline
\multicolumn{1}{|l|}{$R^2_{\mathrm{adj}}$} & \multicolumn{1}{c|}{12.23} & \multicolumn{1}{c|}{22.49} & \multicolumn{1}{c|}{44.83} & \multicolumn{1}{c|}{0.00} & \multicolumn{1}{c|}{0.00} & \multicolumn{1}{c|}{99.99} & \multicolumn{1}{c|}{97.85} & \multicolumn{1}{c|}{4.01} & \multicolumn{1}{c|}{61.26} & \multicolumn{1}{c|}{26.06} & \multicolumn{1}{c|}{26.06} & \multicolumn{1}{c|}{26.06} & \multicolumn{1}{c|}{3.12} & \multicolumn{1}{c|}{2.31} & \multicolumn{1}{c|}{3.71} & \multicolumn{1}{c|}{0.88} & \multicolumn{1}{c|}{0.52} & \multicolumn{1}{c|}{35.96} & \multicolumn{1}{c|}{36.03} & \multicolumn{1}{c|}{36.03} & \multicolumn{1}{c|}{1.62} & \multicolumn{1}{c|}{3.96} & \multicolumn{1}{c|}{3.51} & \multicolumn{1}{c|}{26.06} \\ \hline
\end{tabular}
\end{table*}
\end{comment}

\begin{table*}[]
\setlength{\tabcolsep}{20pt}
\renewcommand{\arraystretch}{1.2}
  \centering
  \scriptsize
  \caption{Model parameters for nonspeech blanking intervention.}
  \vspace{-0.15cm}
  \label{tab:interventionblanking}
  \setlength{\tabcolsep}{0.3em}
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|}
\cline{2-25}
\multicolumn{1}{l|}{} & \multicolumn{12}{c|}{\textbf{GMM}} & \multicolumn{12}{c|}{\textbf{AASIST+RawBoost}} \\ \hline
\multicolumn{1}{|l|}{Params.} & \multicolumn{1}{c|}{\textbf{O}} & \multicolumn{1}{c|}{\textbf{I}} & \multicolumn{1}{c|}{$\textbf{M}_{\mathrm{tr}}$} & \multicolumn{1}{c|}{$\textbf{M}_{\mathrm{te}}$} & \multicolumn{1}{c|}{$\textbf{IT}_{\mathrm{b}}$} & \multicolumn{1}{c|}{$\textbf{IT}_{\mathrm{s}}$} & \multicolumn{1}{c|}{$\textbf{IV}_{\mathrm{bs}}$} & \multicolumn{1}{c|}{$\textbf{IV}_{\mathrm{sb}}$} & \multicolumn{1}{c|}{$\textbf{O}_{\mathrm{s}}$} & \multicolumn{1}{c|}{$\textbf{O}_{\mathrm{b}}$} & \multicolumn{1}{c|}{$\textbf{I}_{\mathrm{s}}$} & $\textbf{I}_{\mathrm{b}}$ & \multicolumn{1}{c|}{\textbf{O}} & \multicolumn{1}{c|}{$\textbf{I}$} & \multicolumn{1}{c|}{$\textbf{M}_{\mathrm{tr}}$} & \multicolumn{1}{c|}{$\textbf{M}_{\mathrm{te}}$} & \multicolumn{1}{c|}{$\textbf{IT}_{\mathrm{b}}$} & \multicolumn{1}{c|}{$\textbf{IT}_{\mathrm{s}}$} & \multicolumn{1}{c|}{$\textbf{IV}_{\mathrm{bs}}$} & \multicolumn{1}{c|}{$\textbf{IV}_{\mathrm{sb}}$} & \multicolumn{1}{c|}{$\textbf{O}_{\mathrm{s}}$} & \multicolumn{1}{c|}{$\textbf{O}_{\mathrm{b}}$} & \multicolumn{1}{c|}{$\textbf{I}_{\mathrm{s}}$} & $\textbf{I}_{\mathrm{b}}$ \\ \hline
\multicolumn{1}{|l|}{$\mu$} & -0.05 & -0.23 & -0.32 & 0.95 & -0.49 & 0.95 & -0.16 & 0.17 & 1.02 & -0.15 & -0.24 & -0.31 & -3.53 & -2.95 & -3.00 & -3.43 & -3.87 & -3.42 & -3.82 & -2.33 & -3.46 & -3.49 & -2.98 & -2.97 \\ \hline
\multicolumn{1}{|l|}{d} & 1.16 & 1.28 & 1.44 & 1.61 & 1.54 & -0.03 & 1.32 & 2.23 & 0.02 & 2.53 & 1.38 & 1.34 & 7.92 & 7.70 & 7.80 & 7.58 & 8.57 & 6.74 & 8.44 & 1.08 & 7.84 & 7.67 & 7.78 & 7.72 \\ \hline
\multicolumn{1}{|l|}{$\beta^{\text{spf}}_\ell$}  & -4.26 & -0.85 & -0.58 & -52.11 & -1.82 & -70.17 & 16.78 & -2.84 & -52.47 & -3.78 & -0.86 & -0.57 & -2.87 & -0.22 & -0.08 & -3.47 & -0.52 & -6.00 & -0.41 & -0.16 & -3.41 & -2.94 & -0.17 & -0.13 \\ \hline
\multicolumn{1}{|l|}{$\beta^{\text{bona}}_\ell$}  & 5.49 & 0.47 & 1.51 & -2.45 & 15.70 & 73.85 & -18.14 & -65.52 & 53.71 & -50.30 & 1.76 & 0.22 & 5.09 & 2.35 & 2.19 & 5.81 & 2.52 & 10.16 & 2.03 & 5.03 & 5.65 & 5.25 & 2.29 & 2.25 \\ \hline
\multicolumn{1}{|l|}{$\sigma$}& 1.49 & 0.64 & 0.61 & 11.69 & 1.40 & 12.41 & 2.95 & 7.43 & 9.95 & 6.31 & 0.60 & 0.65 & 1.36 & 1.25 & 1.25 & 1.36 & 1.39 & 1.79 & 1.44 & 1.84 & 1.35 & 1.36 & 1.25 & 1.25 \\ \hline
\multicolumn{1}{|l|}{$\nu_\mu$} & 0.41 & 0.36 & 0.34 & 0.28 & 0.64 & 0.02 & 0.26 & 0.88 & 0.11 & 0.94 & 0.35 & 0.36 & 0.92 & 0.69 & 0.74 & 0.86 & 0.91 & 0.38 & 0.85 & 0.77 & 0.89 & 0.88 & 0.73 & 0.69 \\ \hline
\multicolumn{1}{|l|}{$\nu_\ell$} & 0.45 & 0.51 & 0.46 & 2.31 & 1.46 & 0.65 & 0.33 & 3.83 & 0.58 & 3.73 & 0.47 & 0.50 & 1.74 & 1.13 & 1.17 & 1.64 & 1.79 & 1.12 & 1.80 & 1.66 & 1.65 & 1.73 & 1.15 & 1.15 \\ \hline
\multicolumn{1}{|l|}{$\upsilon_\mu$} & 1.11 & 1.33 & 1.50 & 1.22 & 2.02 & 1.04 & 1.51 & 1.24 & 1.27 & 1.08 & 1.33 & 1.50 & 1.59 & 1.69 & 1.69 & 1.58 & 1.66 & 2.17 & 1.63 & 1.92 & 1.58 & 1.59 & 1.69 & 1.69 \\ \hline
\multicolumn{1}{|l|}{$\upsilon_\ell$}& 10.91 & 1.42 & 2.51 & 4.17 & 3.91 & 2.03 & 3.82 & 12.83 & 4.18 & 10.80 & 1.42 & 2.51 & 4.35 & 2.71 & 2.73 & 4.40 & 3.00 & 5.53 & 2.89 & 3.99 & 4.39 & 4.35 & 2.71 & 2.72 \\ \hline
\end{tabular}
\vspace{-0.2cm}
\end{table*}


==> tables/intervention_snr.tex <==
\begin{comment}
    
\begin{table*}[]
  \scriptsize
  \caption{Model parameters for additive noise intervention.}
  \label{tab:interventionsnr}
  \setlength{\tabcolsep}{0.5em}
\begin{tabular}{l|cccccccccccc|cccccccccccc|}
\cline{2-25}
 & \multicolumn{12}{c|}{\textbf{GMM}} & \multicolumn{12}{c|}{\textbf{AASIST+RawBoost}} \\ \hline
\multicolumn{1}{|l|}{Params.} & \multicolumn{1}{c|}{\textbf{O}} & \multicolumn{1}{c|}{\textbf{I}} & \multicolumn{1}{c|}{$\textbf{M}_{tr}$} & \multicolumn{1}{c|}{$\textbf{M}_{te}$} & \multicolumn{1}{c|}{$\textbf{IT}_{b}$} & \multicolumn{1}{c|}{$\textbf{IT}_{s}$} & \multicolumn{1}{c|}{$\textbf{IV}_{bs}$} & \multicolumn{1}{c|}{$\textbf{IV}_{sb}$} & \multicolumn{1}{c|}{$\textbf{O}_{s}$} & \multicolumn{1}{c|}{$\textbf{O}_{b}$} & \multicolumn{1}{c|}{$\textbf{I}_{s}$} & $\textbf{I}_{b}$ & \multicolumn{1}{c|}{\textbf{O}} & \multicolumn{1}{c|}{$\textbf{I}$} & \multicolumn{1}{c|}{$\textbf{M}_{tr}$} & \multicolumn{1}{c|}{$\textbf{M}_{te}$} & \multicolumn{1}{c|}{$\textbf{IT}_{b}$} & \multicolumn{1}{c|}{$\textbf{IT}_{s}$} & \multicolumn{1}{c|}{$\textbf{IV}_{bs}$} & \multicolumn{1}{c|}{$\textbf{IV}_{sb}$} & \multicolumn{1}{c|}{$\textbf{O}_{s}$} & \multicolumn{1}{c|}{$\textbf{O}_{b}$} & \multicolumn{1}{c|}{$\textbf{I}_{s}$} & $\textbf{I}_{b}$ \\ \hline
\multicolumn{1}{|l|}{$\mu$} & \multicolumn{1}{c|}{-0.62}	&\multicolumn{1}{c|}{-0.09}	&\multicolumn{1}{c|}{-0.86}	&\multicolumn{1}{c|}{-0.77}&	\multicolumn{1}{c|}{-18.86}&	\multicolumn{1}{c|}{-2.16}&	\multicolumn{1}{c|}{10.89}&	\multicolumn{1}{c|}{17.35}&	\multicolumn{1}{c|}{-0.77}&	\multicolumn{1}{c|}{-0.62}&	\multicolumn{1}{c|}{-0.09}&	\multicolumn{1}{c|}{-0.86}& \multicolumn{1}{c|}{-3.81}&	\multicolumn{1}{c|}{-2.47}&	\multicolumn{1}{c|}{-2.62}&	\multicolumn{1}{c|}{-4.63}&	\multicolumn{1}{c|}{-4.47}&	\multicolumn{1}{c|}{-5.12}&	\multicolumn{1}{c|}{6.22}&	\multicolumn{1}{c|}{6.31}&	\multicolumn{1}{c|}{-4.63}&	\multicolumn{1}{c|}{-3.81}&	\multicolumn{1}{c|}{-2.47}	&\multicolumn{1}{c|}{-2.62} \\ 
\hline
\end{tabular}    
\end{table*}
\end{comment}

\begin{table*}[]
\setlength{\tabcolsep}{20pt}
\renewcommand{\arraystretch}{1.2}
  \scriptsize
  \caption{Model parameters for additive noise intervention.}
  \vspace{-0.15cm}
  \label{tab:interventionsnr}
  \setlength{\tabcolsep}{0.3em}
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|}
\cline{2-25}
\multicolumn{1}{l|}{} & \multicolumn{12}{c|}{\textbf{GMM}} & \multicolumn{12}{c|}{\textbf{AASIST+RawBoost}} \\ \hline
\multicolumn{1}{|l|}{Params.} & \multicolumn{1}{c|}{\textbf{O}} & \multicolumn{1}{c|}{\textbf{I}} & \multicolumn{1}{c|}{$\textbf{M}_{\mathrm{tr}}$} & \multicolumn{1}{c|}{$\textbf{M}_{\mathrm{te}}$} & \multicolumn{1}{c|}{$\textbf{IT}_{\mathrm{b}}$} & \multicolumn{1}{c|}{$\textbf{IT}_{\mathrm{s}}$} & \multicolumn{1}{c|}{$\textbf{IV}_{\mathrm{bs}}$} & \multicolumn{1}{c|}{$\textbf{IV}_{\mathrm{sb}}$} & \multicolumn{1}{c|}{$\textbf{O}_{\mathrm{s}}$} & \multicolumn{1}{c|}{$\textbf{O}_{\mathrm{b}}$} & \multicolumn{1}{c|}{$\textbf{I}_{\mathrm{s}}$} & $\textbf{I}_{\mathrm{b}}$ & \multicolumn{1}{c|}{\textbf{O}} & \multicolumn{1}{c|}{$\textbf{I}$} & \multicolumn{1}{c|}{$\textbf{M}_{\mathrm{tr}}$} & \multicolumn{1}{c|}{$\textbf{M}_{\mathrm{te}}$} & \multicolumn{1}{c|}{$\textbf{IT}_{\mathrm{b}}$} & \multicolumn{1}{c|}{$\textbf{IT}_{\mathrm{s}}$} & \multicolumn{1}{c|}{$\textbf{IV}_{\mathrm{bs}}$} & \multicolumn{1}{c|}{$\textbf{IV}_{\mathrm{sb}}$} & \multicolumn{1}{c|}{$\textbf{O}_{\mathrm{s}}$} & \multicolumn{1}{c|}{$\textbf{O}_{\mathrm{b}}$} & \multicolumn{1}{c|}{$\textbf{I}_{\mathrm{s}}$} & $\textbf{I}_{\mathrm{b}}$ \\ \hline
\multicolumn{1}{|l|}{$\mu$} & -1.04 & -0.08 & -0.91 & -1.24 & -19.27 & -1.35 & 10.94 & 17.35 & -1.26 & -1.01 & -0.07 & -0.93 & -3.87 & -2.61 & -2.64 & -4.82 & -4.61 & -5.51 & 6.28 & 6.37 & -5.10 & -3.73 & -2.58 & -2.58 \\ \hline
\multicolumn{1}{|l|}{d} & 2.90 & 0.44 & 0.30 & 1.41 & 26.07 & 18.99 & -28.15 & -21.92 & 3.04 & 1.24 & -0.51 & 1.24 & 9.48 & 5.96 & 6.42 & 9.27 & 11.34 & 14.51 & -11.52 & -10.80 & 10.57 & 8.17 & 6.36 & 6.36 \\ \hline
\multicolumn{1}{|l|}{$\beta^{\text{spf}}_\ell$} & 0.06 & -0.02 & 0.02 & -0.75 & 0.09 & 2.07 & 0.96 & 0.09 & -0.75 & 0.06 & -0.02 & 0.02 & -0.06 & -0.04 & -0.13 & -0.83 & 0.01 & 0.07 & -0.01 & 0.04 & -0.67 & -0.10 & -0.05 & -0.05 \\ \hline
\multicolumn{1}{|l|}{$\beta^{\text{bona}}_\ell$} & -0.30 & 0.46 & 0.33 & 0.48 & 2.60 & -1.79 & -0.74 & 1.46 & 0.59 & -0.32 & 0.45 & 0.48 & -0.17 & 1.38 & -0.35 & 2.47 & -0.18 & -0.03 & 0.01 & 0.01 & 0.71 & 1.75 & -0.42 & -0.42 \\ \hline
\multicolumn{1}{|l|}{$\sigma$} & 1.61 & 0.28 & 0.67 & 0.48 & 4.57 & 3.60 & 4.42 & 3.19 & 0.48 & 1.61 & 0.32 & 0.66 & 1.41 & 1.18 & 1.17 & 1.03 & 0.75 & 0.75 & 1.07 & 1.28 & 1.03 & 1.40 & 1.19 & 1.19 \\ \hline
\multicolumn{1}{|l|}{$\nu_\mu$} & 0.29 & 0.11 & 0.25 & 0.21 & 5.79 & 1.02 & 0.83 & 4.58 & 0.22 & 0.29 & 0.16 & 0.20 & 0.77 & 0.46 & 0.47 & 0.92 & 0.74 & 0.63 & 0.48 & 1.52 & 0.92 & 0.57 & 0.43 & 0.43 \\ \hline
\multicolumn{1}{|l|}{$\nu_\ell$} & 0.10 & 0.04 & 0.03 & 0.08 & 0.03 & 0.11 & 0.14 & 0.01 & 0.08 & 0.09 & 0.06 & 0.03 & 0.14 & 0.17 & 0.03 & 0.24 & 0.01 & 0.06 & 0.03 & 0.00 & 0.58 & 0.11 & 0.24 & 0.24 \\ \hline
\multicolumn{1}{|l|}{$\upsilon_\mu$} & 2.97 & 0.29 & 0.65 & 0.94 & 4.00 & 2.47 & 4.48 & 2.77 & 0.94 & 2.71 & 0.29 & 0.65 & 1.61 & 1.24 & 1.33 & 2.40 & 0.72 & 0.55 & 0.69 & 1.12 & 2.40 & 1.61 & 1.24 & 1.24 \\ \hline
\multicolumn{1}{|l|}{$\upsilon_\ell$}& 0.15 & 0.28 & 0.14 & 0.32 & 5.05 & 0.46 & 1.66 & 3.84 & 0.32 & 0.15 & 0.28 & 0.15 & 0.24 & 0.25 & 0.62 & 0.66 & 1.28 & 0.05 & 0.07 & 1.75 & 0.66 & 0.24 & 0.26 & 0.26 \\ \hline
\end{tabular}
\vspace{-0.2cm}
\end{table*}

